FloorNet: A Unified Framework for Floorplan Reconstruction from 3D Scans

The ultimate goal of this indoor mapping research is to automatically reconstruct a floorplan simply by walking through a house with a smartphone in a pocket. This paper tackles this problem by proposing FloorNet, a novel deep neural architecture. The challenge lies in the processing of RGBD streams spanning a large 3D space. FloorNet effectively processes the data through three neural network branches: 1) PointNet with 3D points, exploiting the 3D information; 2) CNN with a 2D point density image in a top-down view, enhancing the local spatial reasoning; and 3) CNN with RGB images, utilizing the full image information. FloorNet exchanges intermediate features across the branches to exploit the best of all the architectures. We have created a benchmark for floorplan reconstruction by acquiring RGBD video streams for 155 residential houses or apartments with Google Tango phones and annotating complete floorplan information. Our qualitative and quantitative evaluations demonstrate that the fusion of three branches effectively improves the reconstruction quality. We hope that the paper together with the benchmark will be an important step towards solving a challenging vector-graphics reconstruction problem. Code and data are available at https://github.com/art-programmer/FloorNet.

==> macros.tex <==
% require xspace, array

%% layout
% \newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
% \newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
% \newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

% \newcommand{\xpar}[1]{\noindent\textbf{#1}\ \ }
% \newcommand{\vpar}[1]{\vspace{3mm}\noindent\textbf{#1}\ \ }

% \newcommand{\specialcell}[2][c]{\begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}

%% notations
\newcommand{\sect}[1]{Section~\ref{#1}}
\newcommand{\ssect}[1]{\S~\ref{#1}}
\newcommand{\eqn}[1]{Equation~\ref{#1}}
\newcommand{\fig}[1]{Fig.~\ref{#1}}
\newcommand{\tbl}[1]{Table~\ref{#1}}

\newcommand{\degree}{\ensuremath{^\circ}\xspace}
\newcommand{\ignore}[1]{}
\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\fcseven}{$\mbox{fc}_7$}

\renewcommand*{\thefootnote}{\fnsymbol{footnote}}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

\def\naive{na\"{\i}ve\xspace}
\def\Naive{Na\"{\i}ve\xspace}

\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
%\def\etal{\emph{et al}\onedot}
\def\aka{a.k.a\onedot}
\makeatother

%% comments
\definecolor{MyDarkBlue}{rgb}{0,0.08,1}
\definecolor{MyDarkGreen}{rgb}{0.02,0.6,0.02}
\definecolor{MyDarkRed}{rgb}{0.8,0.02,0.02}
\definecolor{MyDarkOrange}{rgb}{0.40,0.2,0.02}
\definecolor{MyPurple}{RGB}{111,0,255}
\definecolor{MyRed}{rgb}{1.0,0.0,0.0}
\definecolor{MyGold}{rgb}{0.75,0.6,0.12}
\definecolor{MyDarkgray}{rgb}{0.66, 0.66, 0.66}

\newcommand{\jw}[1]{\textcolor{MyDarkGreen}{[Jiajun: #1]}}

\def\bR{\mathbb{R}}
\def\cL{\mathcal{L}}

\newcommand{\z}{\mathbf{z}}
\newcommand{\myparagraph}[1]{\vspace{-13pt}\paragraph{#1}}
\newcommand{\myitem}{\vspace{-7pt}\item}

\newcommand{\presec}{\vspace{-5pt}}
\newcommand{\postsec}{\vspace{-2pt}}
\newcommand{\pressec}{\vspace{-2pt}}
\newcommand{\postssec}{\vspace{-2pt}}

%\newcommand{\mysubsubsubsection}[1]{\vspace{0.1cm} \noindent {\bf #1}:}

==> packages.tex <==
% basic
\usepackage{color,xcolor}
\usepackage{epsfig}
\usepackage{graphicx}

% figure and table
\usepackage{adjustbox}
\usepackage{array}
\usepackage{booktabs}
\usepackage{colortbl}
\usepackage{float,wrapfig}
\usepackage{hhline}
\usepackage{multirow}
\usepackage{subcaption} % issues a warning with CVPR/ICCV format
\usepackage[font={small}]{caption} % fix the font size of tables/figures with CVPR/ICCV format
\captionsetup{compatibility=false}

% font and character
\let\proof\relax
\let\endproof\relax
\usepackage{amsmath,amsfonts,amsthm,amssymb}
\usepackage{bm}
\usepackage{nicefrac}
\usepackage{microtype}

% layout
\usepackage{changepage}
\usepackage{extramarks}
\usepackage{fancyhdr}
\usepackage{lastpage}
\usepackage{setspace}
\usepackage{soul}
\usepackage{xspace}

% ref
\usepackage{url}

% misc
\usepackage{algorithm, algorithmic}
\usepackage{enumerate}
%\usepackage{todonotes} % conflict with CVPR/ICCV format


==> text/5_todo.tex <==
\section{TODO}
\subsection{Does each dataset help?}
python train.py --hybrid=1 --branches=0123 --augmentation=wsf
corner: 0.95 0.54, opening corner: 0.91 0.53, icon corner: 0.85 0.45, room: 0.66 0.36, icon: 0.70, 0.27

python train.py --hybrid=12 --branches=0123 --augmentation=wsf
corner: 0.90 0.50, icon corner: 0.81 0.44, icon: 0.74, 0.23

python train.py --hybrid=13 --branches=0123 --augmentation=wsf
icon corner: 0.83 0.42, icon: 0.74, 0.26

\begin{center}
\begin{tabular}{l|c|c|c}
\hline
 & corner & icon & room\\\hline
Hybrid 01 & 84.9/63.6 & 52.3/25.4 & 62.1/26.5\\
\hline
Hybrid 12 & 87.4/44.7 & 26.1/19.4 & 52.1/23.7\\
\hline
Hybrid 13 & 82.0/49.0 & 42.7/27.8 & 44.1/25.4\\
\hline
Hybrid 14 & 90.4/50.5 & 49.7/23.7 & 61.9/31.6\\
\hline
\end{tabular}
\end{center}

\subsection{Does each augmentation help?}
python train.py --hybrid=1* --branches=0123 --augmentation=ws/wf/sf
python train.py --hybrid=1* --branches=0123 --augmentation=(wsfd)

\begin{center}
\begin{tabular}{l|c|c|c}
\hline
 & corner & icon & room\\\hline
Augmentation  & 77.0/44.9 & 23.7/16.8 & 52.4/23.0\\
\hline
Augmentation sf & 93.7/56.6 & 65.2/30.1 & 65.4/34.1\\
\hline
Augmentation wsf & 93.3/57.9 & 65.8/28.8 & 63.8/38.3\\
\hline
\end{tabular}
\end{center}

\subsection{Does each branch help}
python train.py --hybrid=01234 --branches=* --augmentation=wsf

\begin{center}
\begin{tabular}{l|c|c|c}
\hline
 & corner & icon & room\\\hline
Branch 1 & 90.4/58.2 & 59.0/28.7 & 64.8/34.9\\
\hline
Branch 01 & 93.7/56.7 & 68.8/29.8 & 67.0/39.8\\
\hline
Branch 012 & 95.0/55.1 & 68.4/30.3 & 64.7/38.6\\
\hline
Branch 0123 & 93.3/57.9 & 65.8/28.8 & 63.8/38.3\\
\hline
Branch 01234 & 94.6/53.2 & 66.5/29.2 & 68.3/37.3\\
\hline
\end{tabular}
\end{center}
\subsection{1024}


\begin{center}
\begin{tabular}{l|c|c|c|c|c}
\hline
 & wall corner & opening corner & icon corner & icon & room\\ \hline
Branch 1 & 90.4/58.2 & 87.1/62.0 & 71.8/52.5 & 59.0/28.7 & 64.8/34.9\\
\hline
Branch 01 & 93.7/56.7 & 90.5/63.7 & 80.8/50.7 & 68.8/29.8 & 67.0/39.8\\
\hline
Branch 012 & 95.0/55.1 & 93.9/59.0 & 81.4/51.8 & 68.4/30.3 & 64.7/38.6\\
\hline
Branch 0123 & 93.3/57.9 & 92.0/59.3 & 79.5/52.8 & 65.8/28.8 & 63.8/38.3\\
\hline
Branch 01234 & 94.6/53.2 & 92.0/59.7 & 85.4/52.8 & 66.5/29.2 & 68.3/37.3\\
\hline
\end{tabular}
\end{center}
